An Economic Study of the Effect of Android Platform Fragmentation on Security Updates

Vendors in the Android ecosystem typically customize their devices by modifying Android Open Source Project (AOSP) code, adding in-house developed proprietary software, and pre-installing third-party applications. However, research has documented how various security problems are associated with this customization process. We develop a model of the Android ecosystem utilizing the concepts of game theory and product differentiation to capture the competition involving two vendors customizing the AOSP platform. We show how the vendors are incentivized to differentiate their products from AOSP and from each other, and how prices are shaped through this differentiation process. We also consider two types of consumers: security-conscious consumers who understand and care about security, and na\"ive consumers who lack the ability to correctly evaluate security properties of vendor-supplied Android products or simply ignore security. It is evident that vendors shirk on security investments in the latter case. Regulators such as the U.S. Federal Trade Commission have sanctioned Android vendors for underinvestment in security, but the exact effects of these sanctions are difficult to disentangle with empirical data. Here, we model the impact of a regulator-imposed fine that incentivizes vendors to match a minimum security standard. Interestingly, we show how product prices will decrease for the same cost of customization in the presence of a fine, or a higher level of regulator-imposed minimum security.

==> changes.tex <==

\newcommand{\review}[1]{\vspace{0.5em} \noindent\underline{Comment:} \textit{#1} \vspace{0.5em}}
\newcommand{\response}[1]{\vspace{0.5em} \noindent\underline{Response:} #1 \vspace{0.5em}}


We thank the reviewers for the time that they dedicated to reviewing the earlier version of our paper.
We appreciate their comments, which helped us to significantly improve our paper.
Please find below a list of the reviewer's major comments and how we revised the paper in response to them.

\subsection{Review 1}

%``A paper exploring why Android OEMs don't care about security much. The authors develop a model of Google and an OEM behave and how a regulator might affect OEM behaviour if it fines OEMs who are negligent.''

%``Vendors who customise more can reap more of the benefits of product differentiation but at the cost of security as they introduce new flaws or find it inconvenient to follow Android patches. In a world where customers have imperfect information about security. The authors use a quadratic cost function for the patch quality of customised software and a Hotelling model of consumer knowledge of / preference for security. There is a long and complicated argument that the vendor doesn't invest in security issues arising from customisation, spread over several pages of convexity arguments with partial derivatives. It turns out that a fine can fix this and there's an argument that prices might actually then fall. It could well be true; if the fine is a large enough multiple of the benefit the vendor would get by customising so much that it reduces security past some threshold, then vendors won't go past that, and as a result they won't be able to sell as expensive and mega-customise!''

\review{``But what is the utility of this analysis (given that vendors would game the system in other ways) and can the argument be made more simply?''}

\response{The primary utility of our analysis is providing guidance for regulators. We have made this more clear in the revised paper.
We also provide a more detailed background section on technical work to measure security differentiation (Section~\ref{sec:BackG}). But to the best of our knowledge, no framework exists which allows regulators to reason about these empirical observations. 

Further, we included numerical analysis based on real-world data, which showcases how our model can be applied to study the effects of regulation (Sections~\ref{sec:Num} and~\ref{sec:NumiLL}). Our numerical analysis also gives guidance on how the parameters of our model can be instantiated with real-world data (Section~\ref{sec:NumiLL}).} 

\subsection{Review 2}

%``This is a high level game-theoretic study of the state of Android security by looking at incentives of vendors to customize Google's Android and keeping it up-to-date and secure. The paper confirms the sad state of reality. In short, customization may introduce vulnerabilities, and vendors have incentives to differentiate their products, as follows from general results in this space. The paper formulates a model showing that more customization without proper security is rational for the vendors.''

%``Introducing regulation and fines for too obviously insecure phones has been proposed as a remedy. The paper also analyses this measure and concludes that it indeed has a positive effect on the security level.''


\review{``The start of the paper is interesting to read but the main part mostly consists of less appealing formal derivation of the equilibria.''}

\response{Following the reviewer's advice, we have moved the formal derivations into the appendix.}


\review{``The model assumes that Google also customizes the OS to their hardware ($b > 0$) - is this really the case? why is this necessary?''}

\response{In the revised paper, base Android (i.e., the AOSP version) is assumed to be at the center of customization space (i.e., assumed to be the uncustomized version). In practice, Google actually customizes the software shipped on its devices compared to AOSP~\cite{wu2013impact}. From this perspective, Google may be modeled as just another vendor.}

\review{``I found another implicit assumption more limiting: why is it not possible for a vendor to \emph{increase} the base security? Please explain this choice. In Linux for example, some distributions are more conservative and security-oriented than others. Most vendors enhance the security for their distributions, perhaps by a conservative upgrade strategy (Debian) or dedicated security patches (Ubuntu). I understand this was left out for simplicity but it should be discussed.''}

\response{Studies show that the vast majority of customized Android versions shipped by major vendors are less secure than base Android~\cite{Thomas15}. Consequently, we focus in this paper on the typical vendor attitude, which is to shirk security. We leave the analysis of vendors increasing security for future work.}

%``In Section 5 (Theorem 1) can you give some intuition why the price also increases for Google, even though it does not pay any fines?''

%``Why are there only lemmas in sec. 4 and only theorems in sec. 5?''

%``The paper is an interesting start for modeling the security market of a mobile OS with vendor customization, but leaves out many extra aspects and open to further exploration. Overall this could be an interesting addition to the program.''

\review{``The paper should be proof-read again, sometimes words are missing.''}

\response{We thank the reviwer for providing a list of typos in the review. We have carefully proof read and revised the paper.}

%\todo[inline]{Check the ones below, and say that we proof-read the paper again!}

%``sec. 2, In the previous section ... most closely +related+ research''

%``sec. 4, Our goal is to calculate +the+ Nash equilibrium''

%``sec. 4 a user's preference is +the+ same for both''

\subsection{Review 3}

%``The authors propose a game-theoretic model to try to model Android vendor strategy. The model is inspired by Hotelling's price differentiation model, the twist here is that vendors also pay a premium for implementing security. The takeaways from the model are that vendors have no incentive to implement security, but fines would be an effective incentive, and would not lead to higher overall prices.''

\review{``There is a lot to like in the general problem framing. It is timely, important, especially in light of FTC action, and very relevant to this conference. The mathematical derivations are competently done, and the results are plausible considering the model chosen.''}

\review{``The paper however left me quite unsatisfied. Like many economic models, the outcome is completely dependent on the modeling choices, and those are not particularly well justified here. For instance, in the absence of fines, the utility of each vendor is always decreasing in $q_i$ (the level of security implemented). Then, the authors present the result that vendors do not have any incentive to implement security features: of course not, since they were solely built as a penalty in the model!''}

\response{Following reviewer's suggestion, we extended our model and analysis to consider security-conscious users, who take security level into account when purchasing their phones. In this case, vendors have an incentive to implement security features.}

\review{``I am not sure how you measure the ``level'' of security as a continuous variable, as opposed to a binary value (meets/doesn't meet certain requirements).''}

\response{In practice, the security of smartphones is very often more complex than a binary property. Studies based on real-world data can provide fine-grained quantification of security~\cite{aafer2016harvesting,wu2013impact}.}

\review{``Modeling choices overall are questionable: the authors actually do not model competition between vendors but between one vendor and Google. This is already a bit surprising, because that is not necessarily where I would expect the most merciless competition. Indeed, Google is happy that people use Android as they can monetize the data they get from usage of their services. On the other hand product differentiation between, say, HTC and Samsung, is really where the action is.''}

\response{We have revised the model and analysis in light of the reviewer's suggestion. Now the competition is between vendors.}

%``Even if we buy into the competition model between vendor X and Google, the authors assume that security is not a factor in consumer choice. This is really hard to believe when one of the main selling points of the Nexus/Pixel Google phones is that they are the most secure, patches are always up-to-date, etc. Look at the (recently released) Pixel reviews: they are emphasizing the security aspects as a strong selling point, despite functionality being inferior to some of its competitors'.''

%Had this paper been submitted a few years ago I would have welcomed it with open arms as an interesting use of game theory. However, there have been many such papers, here and at other forums like GameSec, CSF, and by now we expect more, namely, well-motivated models that provide insights. Unfortunately, this paper falls a bit short of that, and
\review{``this paper ... spends most of its page budget in derivations that, however correct, do not yield a lot of insights.''}

\response{We have moved all of the derivations to the appendix in the revised version. We have used the space saved to extend our discussion and provide numerical results based on real-world data.}

%``To be clear, I do not view this as an irredeemable flaw, but it goes beyond mere shepherding, as most of the model justification needs to be rewritten and better motivated, at the very least. Perhaps, the model itself needs tweaking for better generalizability. I recommend the authors revise, and resubmit to a different conference.''



